Applications of deep generative models to DNA reaction kinetics and to cryogenic electron microscopy

This dissertation explores how deep generative models can advance the analysis of challenging biological problems by integrating domain knowledge with deep learning. It focuses on two areas: DNA reaction kinetics and cryogenic electron microscopy (cryo-EM). In the first part, we present ViDa, a biophysics-informed framework leveraging variational autoencoders (VAEs) and geometric scattering transforms to generate biophysically-plausible embeddings of DNA reaction kinetics simulations. These embeddings are reduced to a two-dimensional space to visualize DNA hybridization and toehold-mediated strand displacement reactions. ViDa preserves structure and clusters trajectory ensembles into reaction pathways, making simulation results more interpretable and revealing new mechanistic insights. In the second part, we address key challenges in cryo-EM density map interpretation and protein structure modeling. We provide a comprehensive review and benchmarking of deep learning methods for atomic model building, with improved evaluation metrics and practical guidance. We then present Struc2mapGAN, a generative adversarial network that synthesizes high-fidelity experimental-like cryo-EM density maps from protein structures. Finally, we present CryoSAMU, a structure-aware multimodal U-Net that enhances intermediate-resolution cryo-EM maps by integrating density features with structural embeddings from protein language models via cross-attention. Overall, these contributions demonstrate the potential of deep generative models to interpret DNA reaction mechanisms and advance cryo-EM density map analysis and protein structure modeling.

==> admin_chapters/list_of_abbreviations/list_of_abbreviations.tex <==
\chapter{List of Abbreviations}

% This changes the default spacing of the table. Make sure to reset it to 1 after finished.
\def\arraystretch{1.5}
% The longtable environment allows the table to span multiple pages
\begin{longtable}[l]{l l}
    \textbf{NRCan} & Natural Resources Canada\\
    \textbf{ML} & Machine Learning\\
    \textbf{NN} & Neural Network\\
    \textbf{CNN} & Convolutional Neural Network\\
    \textbf{YCAML} & You Can Add More Lines\\
\end{longtable}
% Reset spacing to default
\def\arraystretch{1}


==> admin_chapters/list_of_symbols/list_of_symbols.tex <==
\chapter{List of Symbols}

% This changes the default spacing of the table. Make sure to reset it to 1 after finished.
\def\arraystretch{1.5}
% The longtable environment allows the table to span multiple pages
\begin{longtable}[l]{l l}
    $c$ & speed of light\\
    $\hbar$ & reduced Planck constant\\
    $\mu_{0}$ & vacuum permeability constant\\
    $\varepsilon_{0}$ & vacuum permittivity constant\\
    $\Delta$ & Laplace operator\\
\end{longtable}
% Reset spacing to default
\def\arraystretch{1}


==> body_chapters/chap_a2/chap_a2.tex <==
% % ------------- VIDA ----------------------

% \chapter{Supplementary Materials for Chapter 2}


% % ------------- Text ----------------------

% \section{Estimated Minimum Passage Time} \label{mfpt}
% $d_{i,j}$ was obtained as the shortest path length between nodes $i,j$, using Dijkstra's algorithm \cite{dijkstra}, on a weighted undirected graph which was constructed in a pre-processing stage from the simulated Multistrand trajectories. In particular, two secondary structure nodes are connected in this graph if at least one of the two possible directions was observed in the training dataset of \emph{elementary transitions}. The edge weight was then chosen to represent the minimum expected holding time between the two adjacent states, where the expected holding time for each state was estimated as the empirical average of the sampled outgoing transition times.

